A Microscopic Perspective on Moir\'e Materials

Contemporary quantum materials research is guided by themes of topology and of electronic correlations. A confluence of these two themes is engineered in "moir\'e materials", an emerging class of highly tunable, strongly correlated two-dimensional (2D) materials designed by the rotational or lattice misalignment of atomically thin crystals. In moir\'e materials, dominant Coulomb interactions among electrons give rise to collective electronic phases, often with robust topological properties. Identifying the mechanisms responsible for these exotic phases is fundamental to our understanding of strongly interacting quantum systems, and to our ability to engineer new material properties for potential future technological applications. In this Review, we highlight the contributions of local spectroscopic, thermodynamic, and electromagnetic probes to the budding field of moir\'e materials research. These techniques have not only identified many of the underlying mechanisms of the correlated insulators, generalized Wigner crystals, unconventional superconductors, moir\'e ferroelectrics, and topological orbital ferromagnets found in moir\'e materials, but they have also uncovered fragile quantum phases that have evaded spatially averaged global probes. Furthermore, we highlight recently developed local probe techniques, including local charge sensing and quantum interference probes, that have uncovered new physical observables in moir\'e materials.

==> Sections/00_KeyPoints.tex <==
\begin{enumerate}
    \item Although many correlated phases in \moire materials were initially discovered by transport measurements, their microscopic nature has been uncovered by a suite of local spectroscopic, thermodynamic, optical, and electromagnetic probes.
    \item The unprecedented tunability of \moire materials has enabled high-resolution spectroscopic and thermodynamic studies of complex translation, rotational, inversion, and time-reversal symmetry-broken phases, many with distinguishable observables to local electromagnetic probes.
    \item Local spectroscopic and phase-sensitive techniques have provided conclusive evidence for unconventional superconductivity in graphene-based \moire materials, and have uncovered remarkable similarities between these platforms and known correlated superconductors.
    \item \Moire materials bring not only promises of advancing our fundamental understanding of exotic quantum phases of matter, but also the potential for novel electronic phases unrealized elsewhere in Nature.
    \item Moreover, the prospects of novel physics and the distinct technological applications of these materials have motivated developing new local probe techniques to access important experimental observables with nano-scale spatial resolution.
\end{enumerate}
